DOD-ETL: Distributed On-Demand ETL for Near Real-Time Business Intelligence

The competitive dynamics of the globalized market demand information on the internal and external reality of corporations. Information is a precious asset and is responsible for establishing key advantages to enable companies to maintain their leadership. However, reliable, rich information is no longer the only goal. The time frame to extract information from data determines its usefulness. This work proposes DOD-ETL, a tool that addresses, in an innovative manner, the main bottleneck in Business Intelligence solutions, the Extract Transform Load process (ETL), providing it in near real-time. DODETL achieves this by combining an on-demand data stream pipeline with a distributed, parallel and technology-independent architecture with in-memory caching and efficient data partitioning. We compared DOD-ETL with other Stream Processing frameworks used to perform near real-time ETL and found DOD-ETL executes workloads up to 10 times faster. We have deployed it in a large steelworks as a replacement for its previous ETL solution, enabling near real-time reports previously unavailable.

==> back.tex <==
\section{Background}
\label{sec:back}

Five fundamental concepts were needed to develop \dod{} and understand the context in which it is founded. The first one, Business Intelligence, refers to the field of expertise related to it. The other two, Distributed Systems and Stream Processing, encompass its core principles. The last two, ETL and CDC, explains the main procedures used by \dod{} to retrieve data from operational databases to be used as input in the decision-making process. 

\subsection{Business Intelligence}

\cite{malhotra2001information} defines Business Intelligence (BI) as a term used to describe a variety of analytical tools that provide easy access to information, which facilitates the decision-making process. These tools range from collecting and consolidating information to analyzing them, enabling analytical capabilities at every level inside and outside a company. 

Within this context, there is the decision-making procedure which, as stated by \cite{aronson2005decision}: ``is a process of choosing among alternative courses of action for the purpose of attaining a goal or goals''. \cite{simon1960new} details this process, breaking it into four phases: intelligence, design, choice, and implementation. 

According to \cite{watson2007current}, BI is a process comprised of two main activities: getting data in and taking it out, where getting data in involves moving data from multiple data sources into the data warehouse. Therefore, this activities extracts and transforms data so that it can be helpful for decision support process. Also, getting data in, which is a responsibility of ETL processes, is the most challenging aspect of BI: ``requiring about 80 percent of the time and effort and generating more than 50 percent of the unexpected project costs''.

Also, despite ETL being the most challenging aspect of BI, it delivers limited value to an enterprise: only when this data is accessed to assist on the decision-making process, it is possible to get value from it.

According to \cite{berson2002building}, among all tools and solutions that comprise BI, there is software to perform: ETL process; data warehousing; database querying and reporting; OLAP data analysis; data mining and data visualization.

Acquiring business insights, as stated by \cite{shari2003business}, implies passing through the process of integrating data from multiples, external and internal, sources, applying tools and techniques to analyze and understand this data and, finally, performing decision-making process based on these insights that were obtained.

\subsection{Distributed Systems}

\cite{tanenbaum2007distributed} define a distributed system as: ``a collection of independent computers that appears to its users as a single coherent system. It consists of components that are autonomous and users think they are dealing with a single system.'' That is, computer heterogeneity and communication differences are kept transparent from the final user on distributed systems, making the interaction with those systems consistent and uniform. 

Having independent computers enables distributed systems to scale relatively easily and to, usually, be continuously available. This reinforces that computer parts replacement or fixing should not be noticeable by the user or the application. 

%In order to support heterogeneous computers and networks while offering a single system view, distributed systems are often organized through a layer of software. That is, logically placed between a higher-level layer consisting of users and applications, and a layer underneath consisting of operating systems and basic communication facilities.

Summing up, according to \cite{tanenbaum2007distributed}, a distributed system should: (1) hide from the user that resources are placed separately across a network, (2) enable resources to be easily accessible and (3) be scalable.

Among the distributed systems, there is an important class, called cluster computing, used for compute-intensive tasks. Its hardware is comprised of a number of similar commodity computers, closely connected by some high-speed network. Its use became more frequent when the ratio between price and performance of these computers started to get lower, reaching the point where off-the-shelf technology can be used to build supercomputers.

\subsection{Stream processing}

\cite{cherniack2003scalable} define stream processing as a class of applications where data, from external source systems, is pushed asynchronously to targets that consume this information. The main characteristic of these applications, also known as stream-based applications, is its timely high-volume data streams processing.

Also, according to \cite{cherniack2003scalable}, database management systems (DBMS) work using a pull-based model for accessing data, in which the user, the one that submits the query, is active and the management system is passive, returning the answer to the query. Opposite to this model, stream-based applications push the query answer to a waiting user or application. Therefore, inverting this data management model, assuming users as passive and data management systems as active. 

\cite{cherniack2003scalable} concludes that, due to the nature of stream-based applications, they are mostly distributed: they are often on environments with multiple interconnected devices and, as data flows from its source point to its target, each of these devices it passes through is a potential target of computation. As expected of a distributed system, more computing devices could be added to the system to handle load changes.

Since a data stream is a potentially unbounded data collection, arriving gradually over time, stream applications process these incoming streams as a data flow, which in turn is modeled as a directed acyclic graph of processing operators. These operators work accepting input streams, applying some transformation to them and producing one or multiple stream outputs. This abstraction allows applications to exploit a form of parallel and distributed processing more easily. 

In this stream-based applications context, multiple stream processing frameworks facilitate the development of such applications. Most of them are based on the record-at-a-time processing model, in which each record is processed independently. Examples of stream processors frameworks that use this model are Yahoo!’s S4 \cite{neumeyer2010s4} and Twitter’s Storm \cite{toshniwal2014storm}. 

In contrast to this record-at-a-time processing model, another possibility is to model it as a series of small deterministic batch computations, as proposed by \cite{zaharia2012discretized}. This way, among others benefits, integration with a batch system is made easy and performance overhead, due to record-at-a-time operations, is avoided.

\subsection{Extract Transform Load}

Integration between transactional and decision support applications are done by a procedure, comprising three steps, known as ETL (Extract Transform Load). As explained in more detail below, those stages are responsible for \textbf{extracting} data from different and heterogeneous sources, \textbf{transforming} it to fit a target schema, which is more appropriate for reporting and analysis and, finally, \textbf{loading} it on the target data warehouse. 

Since it involves large amounts of heterogeneous data, complex operations, integration of multiple data sources, and it is susceptible to numerous problems, it is deemed to be a mission-critical process in BI solutions.

Two processing strategies can be used in ETL process: (1) Batch and (2) Stream processing. The difference between them resides on whether the source system data is bounded (by known and finite size) or unbounded (arrives gradually over time).   

As stated by \cite{kleppmann2017designing}: ``Batch processing techniques read a set of data chunks (bounded data) as input and produce a new set of output. The output is a form of derived data; that is, a dataset that can be recreated by running the batch process again if necessary." This process is done in cycles and, typically, with considerable time between executions.

As already explained in the previous section, stream processing is designed primarily for unbounded data sets, reading data as it is produced and processing it continuously. It is important to point out that, if well-designed, stream processing systems can provide the same features as batch processing, but on \nrt{}. 

The ETL steps are:

\begin{itemize}
\item Extract: this step identifies which portion of the source data should be extracted for further processing, making sure that the source suffers \textbf{minimum overhead} during this step. After new data is identified, it needs to be propagated to the next step (Transform).
\item Transform: considered the core step on the ETL process, it transforms data into the expected format once extracted data is accessible. This transformation involves various operations, like normalizing, summarizing, merging and so forth.
\item Load: after going through the transformation process, data needs to be loaded into the data warehouse. How the data warehouse stores data also influences the loading performance, which, in turn, is related to the technologies and techniques used.
\end{itemize}

\subsection{Change Data Capture}

The extraction stage identifies what data could be submitted to the ETL process, taking care that the source suffers minimum overhead during this step. To do so, this step should submit as little data as possible, detecting only new/altered data.

The set of patterns and techniques used to detect changes in databases is called Change Data Capture (CDC). \cite{vassiliadis2009near} describes some of the techniques to perform CDC extraction:

\begin{itemize}
\item Application Middleware - Applications are equipped with a middleware that sends data as it is altered.
\item Trigger - Triggers are created in the source database to notify on each modification that happens in the source database.
\item Timestamp - Add a column with transaction timestamp and extract, periodically, records with timestamp greater than the last execution. 
\item Log - Analyze transaction log and sends content with the timestamp greater than last execution.
\end{itemize}

As also stated by \cite{vassiliadis2009near}, after new/altered data is identified, it needs to be propagated. There are three technical choices to perform this propagation: periodic, pull-based, in which the consumer request data or (c) push-based, in which the source database sends data at its own pace.

\subsection{Summary}

This chapter made a brief presentation of the concepts underlying \dod{}. These concepts contextualize the reader, introducing the fundamentals behind the proposed solution.

Some works and publications that relate, in some way, to \dod{}, and to \nrt{} ETL will be presented in \strc{sec:rw}. They go from describing the challenges of developing a \nrt{} ETL process to proposing strategies and solutions to address this topic.


